Computer-aided quantization and numerical analysis of superconducting circuits

The development of new superconducting circuits and the improvement of existing ones rely on the accurate modeling of spectral properties which are key to achieving the needed advances in qubit performance. Systematic circuit analysis at the lumped-element level, starting from a circuit network and culminating in a Hamiltonian appropriately describing the quantum properties of the circuit, is a well-established procedure, yet cumbersome to carry out manually for larger circuits. We present work utilizing symbolic computer algebra and numerical diagonalization routines versatile enough to tackle a variety of circuits. Results from this work are accessible through a newly released module of the scqubits package.

==> IPynotebook_preamble.tex <==
%-------
%   Typography
%-------

\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{textcomp}
\usepackage{dsfont}
\usepackage{microtype}
\usepackage[onehalfspacing]{setspace}

%-------
%   Notebook Styling
%-------

\usepackage[most]{tcolorbox}
\tcbuselibrary{listings}
\tcbset{nobeforeafter}

\definecolor{outcolor}{HTML}{D84315}

\newlength{\promptwidth}
\setlength{\promptwidth}{30pt}
\newlength{\promptsep}
\setlength{\promptsep}{5.5pt}

\newcommand{\prompt}[4]{%
    \makebox[0pt][r]{\texttt{\color{#2}#1[#3]:#4}}\vspace{-\baselineskip}%
}

\newcounter{NBin}

\newtcblisting{NotebookOut}{
    breakable,
    boxrule=.5pt,
    size=fbox,
    left skip = \promptwidth + \promptsep,
    pad at break*=1mm,
    opacityfill=1,
    phantom=\refstepcounter{NBin},
    title=\prompt{}{outcolor}{\theNBin}{\hspace{\promptsep}},
    fonttitle=\linespread{1}\small,
    attach title to upper,
    listing only,
    listing options={
        language=python,
        basicstyle=\linespread{1}\ttfamily,
        basewidth=.5em,
        aboveskip=0pt,
        belowskip=0pt,
        showstringspaces=false,
    }
}

==> images/jk_tikz_elec_circuit.tex <==
\makeatletter
% Do not add spurious spaces
\tikzset{jk/.style=
	{%
		% generic tikz-level settings
		cute inductors,%
		%circutikz-level settings
		\circuitikzbasekey/.cd,%
		bipoles/thickness=1.5,
		bipole voltage style/.style={color=red},
		bipole current style/.style={color=blue},
		%bipole flow style/.style={color=red},
		%bipoles/crossing/size=4,
		%
		% Capacitors
		% capacitors/scale=0.7,
		capacitors/thickness=1.2, 
		capacitors/width/.try=0.085,
		capacitors/height/.try=0.3,
		%capacitors/width/.try=0.15, % from 1.4.1 
		%capacitors/height/.try=0.6, % from 1.4.1
		%
		% Inductors (and transformers) 
		inductors/scale=0.9,
		inductors/thickness=1.0,
		inductors/coils=4,
		inductors/width/.try=0.6,
		%inductors/height=0.25,
		% 
		% Ground symbols 
		grounds/scale=0.6, 
		grounds/thickness=1.0,
		%
		% Voltage
		voltage/distance from node=0.0,
		voltage/shift=2.1,
		voltage/bump b=0.7,
		voltage/european label distance=1.2,
		%voltage/american label distance=1.2,
		%voltage/american font=\tiny\boldmath,%
		% other options for romano style
		bipoles/crossing/size=0.4,
		% monopoles/vcc/arrow={Triangle[width=0.8*\scaledwidth, length=\scaledwidth]},
		% monopoles/vee/arrow={Triangle[width=0.8*\scaledwidth, length=\scaledwidth]},
		%
		% Nodes width (connectors, etc
		nodes width=.04, % size of nodes
		%
		% Arrows size
		current arrow scale=16, % smaller is larger arrow
		% Switches 
		bipoles/cuteswitch/thickness,
		%
		% Transmission line 
		bipoles/tline/height=0.5,
		%
		% Logic ports - amp, buffer, etc. 
		logic ports/thickness=4.0,
	},% end .style
}% end \tikzset



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% JJ
\ctikzset{bipoles/jj/height/.initial=.23}
\ctikzset{bipoles/jj/width/.initial=.23}
\ctikzset{bipoles/jj/thickness/.initial=1}

\pgfcircdeclarebipolescaled{inductors}
	{} % extra anchors
	{\ctikzvalof{bipoles/jj/height}} % depth under path line
	{jj} % name 
	{\ctikzvalof{bipoles/jj/height}} % height above path line
	{\ctikzvalof{bipoles/jj/width}}  % width
	{ % code
	    % cross
	    \pgfsetlinewidth{\ctikzvalof{bipoles/jj/thickness}\pgfstartlinewidth}
	    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	    \pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	
	    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	    \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	
	    \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
		\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	    \pgfusepath{draw}
	}

\pgfcirc@activate@bipole@simple{l}{jj}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% JJ bare
\ctikzset{bipoles/jjbare/height/.initial=.2}
\ctikzset{bipoles/jjbare/width/.initial=.2}
\ctikzset{bipoles/jjbare/thickness/.initial=1}

\pgfcircdeclarebipolescaled{inductors}
{} % extra anchors
{\ctikzvalof{bipoles/jjbare/height}} % depth under path line
{jjbare} % name 
{\ctikzvalof{bipoles/jjbare/height}} % height above path line
{\ctikzvalof{bipoles/jjbare/width}}  % width
{ % code
	% cross
	\pgfsetlinewidth{\ctikzvalof{bipoles/jjbare/thickness}\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}}
	
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}}
	\pgfusepath{draw}
	
	% straight wire
	\pgfsetlinewidth{\pgfstartlinewidth}
	\pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
	\pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}    
	\pgfusepath{draw}
}

\pgfcirc@activate@bipole@simple{l}{jjbare}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Spider

\pgfcircdeclarebipolescaled{inductors}
{} % extra anchors
{\ctikzvalof{bipoles/jj/height}} % depth under path line
{spider} % name 
{\ctikzvalof{bipoles/jj/height}} % height above path line
{\ctikzvalof{bipoles/jj/width}} % width
{ % code
   % \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
   \pgfsetlinewidth{\ctikzvalof{bipoles/jj/thickness}\pgfstartlinewidth}

   % left to right acr
   \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}} % start point
   \pgfpathcurveto
    {\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}} % support point 1
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}} % support point 2
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % final point
   \pgfusepath{stroke}

   % right to left acr
   \pgfpathmoveto{\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@up}} % start point
   \pgfpathcurveto
    {\pgfpoint{\pgf@circ@res@left}{\pgf@circ@res@down}} % support point 1
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@up}} % support point 2
    {\pgfpoint{\pgf@circ@res@right}{\pgf@circ@res@down}} % final point
   \pgfusepath{stroke}

   % straight wire
   \pgfsetlinewidth{\pgfstartlinewidth}
   \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
   \pgfpathlineto{\pgfpoint{\pgf@circ@res@left}{0pt}}    
   \pgfusepath{draw}
}

\pgfcirc@activate@bipole@simple{l}{spider}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Snail

\pgfcircdeclarebipolescaled{inductors}
{} % extra anchors
{\ctikzvalof{bipoles/jj/height}} % depth under path line
{snail} % name 
{\ctikzvalof{bipoles/jj/height}} % height above path line
{\ctikzvalof{bipoles/jj/width}} % width
{ % code
   % \pgf@circ@setlinewidth{bipoles}{\pgfstartlinewidth}
   \pgfsetlinewidth{\ctikzvalof{bipoles/jj/thickness}\pgfstartlinewidth}

   \pgfplothandlerlineto   
   \pgfplotfunction{\x}{0,10,...,720}{
      \pgfpointxy{
       \ctikzvalof{bipoles/jj/width} *exp(-0.1*rad(\x))*cos(\x)}{
       \ctikzvalof{bipoles/jj/height}*exp(-0.1*rad(\x))*sin(\x)}}
   \pgfusepath{stroke}

   % straight wire
   \pgfsetlinewidth{\pgfstartlinewidth}
   \pgfpathmoveto{\pgfpoint{\pgf@circ@res@right}{0pt}}
   \pgfpathlineto{\pgfpointxy{
      \ctikzvalof{bipoles/jj/width} *exp(-0.1*rad(360))*cos(360)
   }{0pt}}    
   \pgfusepath{draw}
}

\pgfcirc@activate@bipole@simple{l}{snail}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% American voltage sourse with rotating sign      -
%  https://tex.stackexchange.com/questions/176296/circuitikz-voltage-source-american-style

\pgfcircdeclarebipole{}{\ctikzvalof{bipoles/vsourceam/height}}{vsourceAM}{\ctikzvalof{bipoles/vsourceam/height}}{\ctikzvalof{bipoles/vsourceam/width}}{

    \pgfsetlinewidth{\pgfkeysvalueof{/tikz/circuitikz/bipoles/thickness}\pgfstartlinewidth}

    \pgfpathellipse{\pgfpointorigin}{\pgfpoint{0}{\pgf@circ@res@up}}{\pgfpoint{\pgf@circ@res@left}{0}}
    \pgfusepath{draw}
    \pgfscope
        \pgftransformxshift{\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@left}
        \pgftext[rotate=-\pgf@circ@direction]{$-$}
        \pgfusepath{draw}
    \endpgfscope
    \pgfscope
        \pgftransformxshift{\ctikzvalof{bipoles/vsourceam/margin}\pgf@circ@res@right}
        \pgftext[rotate=-\pgf@circ@direction]{$+$}
        \pgfusepath{draw}
    \endpgfscope
}
\pgfcirc@activate@bipole@simple{l}{vsourceAM}
\ctikzset{bipoles/vsourceam/margin=.5}% default too big - moves plus minus closer in 
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% showcase circ
\newcommand{\thiscirc}[2]{ 
 \texttt{#2} 
 \hfill 
 \begin{circuitikz} 
    \draw (0,0) node[ #1 ] {};  
 \end{circuitikz}
}

